MPGM: Scalable and Accurate Multiple Network Alignment

Protein-protein interaction (PPI) network alignment is a canonical operation to transfer biological knowledge among species. The alignment of PPI-networks has many applications, such as the prediction of protein function, detection of conserved network motifs, and the reconstruction of species' phylogenetic relationships. A good multiple-network alignment (MNA), by considering the data related to several species, provides a deep understanding of biological networks and system-level cellular processes. With the massive amounts of available PPI data and the increasing number of known PPI networks, the problem of MNA is gaining more attention in the systems-biology studies. In this paper, we introduce a new scalable and accurate algorithm, called MPGM, for aligning multiple networks. The MPGM algorithm has two main steps: (i) SEEDGENERATION and (ii) MULTIPLEPERCOLATION. In the first step, to generate an initial set of seed tuples, the SEEDGENERATION algorithm uses only protein sequence similarities. In the second step, to align remaining unmatched nodes, the MULTIPLEPERCOLATION algorithm uses network structures and the seed tuples generated from the first step. We show that, with respect to different evaluation criteria, MPGM outperforms the other state-of-the-art algorithms. In addition, we guarantee the performance of MPGM under certain classes of network models. We introduce a sampling-based stochastic model for generating k correlated networks. We prove that for this model, if a sufficient number of seed tuples are available, the MULTIPLEPERCOLATION algorithm correctly aligns almost all the nodes. Our theoretical results are supported by experimental evaluations over synthetic networks.

==> tex/document.tex <==
In this talk we will consider maximizing a submodular function in a streaming setting.
Submodular functions are an important class of discrete functions with many applications in data summarization.

==> tex/rationale1.tex <==
% !TeX root = MNA.tex



\subsection{Why SeedGeneration?} 

The first step of MROPER (\FuncSty{SeedGeneration}) is a heuristic  algorithm that generates seed-tuples.
\FuncSty{SeedGeneration} is designed  based on the following observations.
First, we know that proteins with high BLAST bit-score  similarities share GO terms with a high probability \citep{joshi2007} and high levels of sequence similarity is often a good indicator of functional similarity between proteins \citep{pesquita2008}. 
See \sref{sec:whyseedgen} for further experimental verifications.
Second, we look at the transitivity of BLAST bit-score similarities for real proteins.
In general, the BLAST similarity is not a transitive measure, i.e., for proteins $p_1, p_2$ and $p_3$ given that couples 
$[p_1, p_2]$ and $[p_2, p_3]$ are similar, we can not always conclude that the two proteins $p_1$ and $p_3$ are similar. 
But real proteins cover a small portion of the space of possible amino-acid 
sequences, and it might be safe to assume a (pseudo) transitivity property for 
them.
\begin{example}
Consider the three toy proteins $p_1, 
p_2$ and $p_3$ with amino-acid sequences $[MMMMMM], [MMMMMMVVVVVV]$ and 
$[VVVVVV]$, respectively. In this example, $p_2$ is similar to both $p_1$ and 
$p_3$, where $p_1$ is not similar to $p_3$. Indeed, we have $BlastBit(p_1 , 
p_2) = 11.2, BlastBit(p_2 , p_3 ) = 10.0$ and $BlastBit(p_1 , p_3) = 0$. 
\end{example}

%  Next, we study the transitivity in the sequence similarities of real 
% proteins. 
To empirically evaluate the transitivity of BLAST bit-scores, we define a new 
measure for an estimation of the BLAST bit-score similarity of two 
proteins $p_1$ and $p_3$, when we know that there is a protein $p_2$, such that 
BLAST bit-score similarities between $p_2$ 
and both $p_1,p_3$ are at least $\ell$. Formally, we define 
$\alpha_{\ell, \beta}$ as
\begin{align*}
\alpha_{\ell, \beta}  = \argmax_{\alpha} \Big[  \mathbb{P} & [BLAST(i,k)   \geq \alpha \times \ell \ |  \\ &\ BLAST(i,j) \geq \ell, BLAST(j,k) \geq \ell ]   \geq \beta \Big]. 
\end{align*}

  
A value of $\alpha_{\ell, \beta}$, which is close to one,
is an indicator of a high level of 
transitivity (with a probability of $\beta$) between the sequence similarities 
of protein couples. 
In Figure~\ref{fig:trans}, we study the transitivity of BLAST bit-scores for 
different levels of confidence $\beta$. 
For example, in this figure, we observe that for two couples $[p_1,p_2]$ and 
$[p_2,p_3]$ with BLAST bit-score similarities of at least $100$, the similarity 
of the couple $[p_1,p_3]$ is at least 91 with a probability of $0.80$. In 
general, based on these experimental evidence, it seems reasonable to assume 
that there is a \textit{pseudo transitive} relationship between the sequence 
similarities of real proteins. 


\begin{figure}[!tpb]
%\begin{center} 
\centering
\includegraphics[width=6.cm, keepaspectratio]{figures/trans.eps}
  \caption{The transitivity of BLAST bit-score similarities for real proteins. 
The $\alpha_{\ell, \beta}$ measure is calculated for different values of 
$\ell$ and $\beta$.} 
\label{fig:trans}
%\end{center}
\end{figure}

%\end{itemize}

The two main observations about (i) the relationship between sequence 
similarity and biological functions of protein couples, and (ii) 
the transitivity 
of BLAST bit-scores help us to design a heuristic algorithm for generating 
high-quality clusters ($\ell$-consistent tuples) from sequence 
similarities. 

\subsection{Why the MultiplePercolation?}

The general class of PGM algorithms has been shown to be very powerful for 
global pairwise-network alignment problems. For example, PROPER is a
state-of-the-art algorithm
that uses PGM-based methods to align two networks \citep{kazemi2016proper}. There 
are several works 
on 
the theoretical and practical aspects of PGM algorithms 
\citep{narayanan:2009,Yartseva:2013,korula14efficient,kazemi2015when,chiasserini2017anonymizing}. 

In this paper, we introduced a global MNA algorithm, as a new  member of the PGM class.
% for multiple global network 
% alignment problem.  
In Supplementary~Section~3, by using a parsimonious $k$-graph sampling model (as a generalization of the model from \citep{kazemi2015when}), we prove that \FuncSty{MultiplePercolation} aligns all the nodes correctly, if initially enough number of seed-tuples are provided (See Supplementary Theorems 1 and 2). 
%We first explain the model. Then we state the main theorem. 
Also, in Supplementary Figures~\ref{fig:pgmk_5_0.9_0.9}, \ref{fig:pgmk_4_0.9_0.9} and \ref{fig:pgmk_3_0.9_0.9} we present experimental evaluations of \FuncSty{MultiplePercolation} over random graphs that are generated based on our $k$-graph sampling model. 
We observe that when there are enough number of tuples in the seed set (which matches exactly to the values given by theorems),  \FuncSty{MultiplePercolation} aligns correctly most of the nodes. We also see the sharp phase-transitions predicted in supplementary theorems.

==> tex/rationale2.tex <==





==> tex/suppl_compare.tex <==
% !TeX root = suppl.tex



\section{Experimental Evaluations}



==> tex/suppl_seedgen.tex <==
\subsection{Why SeedGeneration?} \label{sec:whyseedgen}
The first step of \AlgMPROPER (\AlgSeed) is a heuristic 
algorithm that generates seed-tuples. \AlgSeed is designed 
based on the following observations.
%   \subsubsection{Observations}
%   We make two important observations.
  %\begin{itemize}
   %\item
    First, we argue that proteins with high BLAST bit-score 
similarities share GO terms with a high probability. 
To provide experimental evidence for our hypothesis, we look at the biological 
similarity of protein couples versus their BLAST bit-score similarities.
For this reason, we define a gene-ontology consistency (GOC) measure (based on 
the measure introduced in \cite{mistry2008gene}) to evaluate the 
relationship 
between BLAST bit-scores and the experimentally verified GO terms.
This measure represents the percentage of pairs of proteins with BLAST bit-score
similarity of at least $\ell$, such that they share at least one GO term. 
Formally, we define
\begin{align}
 goc_{\geq \ell} = \dfrac{|\{ [p_i, p_j] | BLAST(p_i, p_j) \geq \ell \text{ and 
} 
go(p_i) \cap go(p_j) \neq \emptyset \}|}{|\{ [p_i, p_j] | BLAST(p_i, p_j) \geq 
\ell, go(p_i) \neq \emptyset \text{ and } 
go(p_j) \neq \emptyset \}|}.
\end{align}
In this section, we consider only experimentally verified GO 
terms. 
% For this 
% reason, we 
% consider the GO terms with codes ``EXP'', ``IDA'', ``IMP'', ``IGI'' and 
% ``IEP'', and we exclude the annotations derived from computational methods and 
% protein-protein interaction experiments.
Figure~\ref{fig:blast_go} shows the $goc_{\geq \ell}$ measure for couples of 
proteins among five eukaryotic species, namely C. elegans (ce), D. melanogaster 
(dm), H. sapiens (hs), M. musculus (mm) and S. cerevisiae (sc).
In this figure, the results are provided for cases, where we consider (i) all 
the experimental GO terms, (ii) cellular component (CC) annotations, 
(iii) molecular function (MF) annotations, and (iv) biological process (BP) 
annotations.
For further experiments, we look at the average of semantic similarity $SS_p$ (main article, Section 2.2, Equation (1)) between couples of proteins with BLAST bit-score similarity of 
at least $\ell$. Figure~\ref{fig:blast_Resnik} shows the $SS_p$ for couples  of 
proteins with 
BLAST bit-score similarities of at least $\ell$. We observe that, for couples 
of proteins with higher BLAST bit-score similarities, the average of $SS_p$ 
measure increases.
%
\begin{figure}[!tpb]
\centering
\includegraphics[width=6cm, keepaspectratio]{figures/goc_acc.eps}
  \caption{The $goc_{\geq \ell}$ measure for couples of proteins with BLAST 
bit-score similarities of at least $\ell$.} 
\label{fig:blast_go}
%\end{center}
\end{figure}
%
\begin{figure}[!tpb]
\centering
\includegraphics[width=6cm, keepaspectratio]{figures/average_resnik.eps}
  \caption{Average of $SS_p$ for couples of proteins with BLAST bit-score 
similarities of at least $\ell$. We observe that, for couples 
of proteins with higher BLAST bit-score similarities, the average of $SS_p$ 
measure increases.} 
\label{fig:blast_Resnik}
%\end{center}
\end{figure}
